Study of JavaScript Static Analysis Tools for Vulnerability Detection in Node.js Packages

With the emergence of the Node.js ecosystem, JavaScript has become a widely-used programming language for implementing server-side web applications. In this paper, we present the first empirical study of static code analysis tools for detecting vulnerabilities in Node.js code. To conduct a comprehensive tool evaluation, we created the largest known curated dataset of Node.js code vulnerabilities. We characterized and annotated a set of 957 vulnerabilities by analyzing information contained in npm advisory reports. We tested nine different tools and found that many important vulnerabilities appearing in the OWASP Top-10 are not detected by any tool. The three best performing tools combined only detect up to 57.6% of all vulnerabilities in the dataset, but at a very low precision of 0.11%. Our curated dataset offers a new benchmark to help characterize existing Node.js code vulnerabilities and foster the development of better vulnerability detection tools for Node.js code.

==> listings/advisory-1147.tex <==
\begin{listing}[t]
% Advisory 1147
\begin{minted}[
    xleftmargin=15pt,
    breaklines,
    breakbytoken,
    linenos,
    fontsize=\scriptsize]{js}
// Snippet of ./simple-markdown.js
var defaultRules = {
    inlineCode: {
        match: inlineRegex(/^(`+)\s*([\s\S]*?[^`])\s*\1(?!`)/),
        parse: function(capture, parse, state) {
            return {
                content: capture[2]
            };
        },
    },
};

var defaultInlineParse = function(source, state) {
    state = state || {};
    state.inline = true;
    return defaultRawParse(source, state);
};
\end{minted}
\vspace{-0.1cm}
\caption{\small ReDoS (advisory 1147) - SNYK-JS-SIMPLEMARKDOWN-460540~\cite{SNYK-JS-SIMPLEMARKDOWN-460540}.}
\label{snippet:advisory-1147}
\vspace{-0.3cm}
\end{listing}

==> listings/advisory-1490.tex <==
\begin{listing}[t]
% Advisory 1490
\begin{minted}[
    xleftmargin=15pt,
    breaklines,
    breakbytoken,
    linenos,
    fontsize=\scriptsize]{js}
// Snippet of ./index.js:
function ctorName(val) { 
    return val.constructor ? val.constructor.name : null; 
}

// Proof-of-Concept exploit code:
var kindOf = require('kind-of');
var user_input = {
    user: 'barney',
    age: 36,
    active: true,
    "constructor":{"name":"Symbol"}
};
console.log(kindOf(user_input)); // "symbol" <== instead of "object"
\end{minted}
\vspace{-0.1cm}
\caption{\small Type Checking Error (advisory 1490) - CVE-2019-20149~\cite{CVE-2019-20149}.}
\label{snippet:advisory-1490}
\vspace{-0.3cm}
\end{listing}

==> listings/advisory-557.tex <==
\begin{listing}[t]
% Advisory 1143
\begin{minted}[
    xleftmargin=15pt,
    breaklines,
    breakbytoken,
    linenos,
    fontsize=\footnotesize]{js}
// Snippet of ./middleware/file_explorer.js:
module.exports = function* (next) {
    const directory = config.get(configKey.DIRECTORY);
    let requestPath = decodeURIComponent(this.request.path);
    let fullRequestPath = path.join(directory, requestPath);
    let stat = yield getFileStat(fullRequestPath);
    if (stat.isDirectory()) {
        let files = yield readFolder(fullRequestPath);
        // (...)
    }
};
\end{minted}
\vspace{-0.1cm}
\caption{\small Path Traversal (advisory 557) - HackerOne Report 296254~\cite{hackerone-296254}: Vulnerable source (line 4) and sink (line 8).}
\label{snippet:advisory-557}
\vspace{-0.3cm}
\end{listing}

==> tables/cwes-onecolumn.tex <==
% \begin{table}[t]
% \centering
% \small
% %\footnotesize
% \begin{tabular}{c|llc}
% \hline
% \textbf{\#} & \textbf{CWE} & \textbf{Security Risk}  & \textbf{\# Occurrences} \\ \hline
% 1 & CWE-22  & 5. Broken Access Control      & 160   \\ 
% 2 & CWE-79  & 7. Cross-Site Scripting       & 132   \\ 
% 3 & CWE-818 & 3. Sensitive Data Exposure    & 123   \\ 
% 4 & CWE-400 & - & 81    \\ 
% 5 & CWE-471 & - & 63    \\ 
% 6 & CWE-78  & 1. Injection                  & 45    \\ 
% 7 & CWE-94  & 1. Injection                  & 34    \\ 
% 8 & CWE-20  & - & 26    \\ 
% 9 & CWE-200 & 3. Sensitive Data Exposure    & 22     \\ 
% 10 & CWE-89 & 1. Injection                  & 20     \\ \hline
% \end{tabular}
% \caption{\small Possible mapping of most occurring vulnerabilities in dataset with OWASP Top 10 Web Security Risks (2017). The CWEs are titled: Path Traversal (CWE-22), Cross-site Scripting (CWE-79), Insufficient Transport Layer Protection (CWE-818), Resource Exhaustion (CWE-400), Modification of Assumed-Immutable Data (CWE-471), OS Command Injection (CWE-78), Code Injection (CWE-94), Improper Input Validation (CWE-20), Exposure of Sensitive Information (CWE-200), and SQL Injection (CWE-89).}
% \label{table:cwes}
% \vspace{-0.1cm}
% \end{table}

\begin{table}[t]
\centering
\small
%\footnotesize
\begin{tabular}{c|llc}
\hline
\textbf{\#} & \textbf{CWE} & \textbf{Security Risk}  & \textbf{\# Occurrences} \\ \hline
1 & CWE-22  & 1. Broken Access Control      & 160   \\ 
2 & CWE-79  & 3. Injection                  & 132   \\ 
3 & CWE-818 & 2. Cryptographic Failures     & 123   \\ 
4 & CWE-400 & -                             & 81    \\ 
5 & CWE-471 & 3. Injection                  & 63    \\ 
6 & CWE-78  & 3. Injection                  & 45    \\ 
7 & CWE-94  & 3. Injection                  & 34    \\ 
8 & CWE-20  & 3. Injection                  & 26    \\ 
9 & CWE-200 & 1. Broken Access Control      & 22     \\ 
10 & CWE-89 & 3. Injection                  & 20     \\ \hline
\end{tabular}
\caption{\small Possible mapping of most occurring vulnerabilities in dataset with OWASP Top 10 Web Security Risks (2021)~\cite{owasp-mapping}. The CWEs are titled: Path Traversal (CWE-22), Cross-site Scripting (CWE-79), Insufficient Transport Layer Protection (CWE-818), Resource Exhaustion (CWE-400), Modification of Assumed-Immutable Data (CWE-471), OS Command Injection (CWE-78), Code Injection (CWE-94), Improper Input Validation (CWE-20), Exposure of Sensitive Information (CWE-200), and SQL Injection (CWE-89).}
\label{table:cwes}
\vspace{-0.1cm}
\end{table}

==> tables/results.tex <==
% Verde acima de 50%
% Amarelo acima de 15%
% Consigo gerar facilmente esta tabela com outras cores para outros valores
\begin{table*}[t]
\centering
\footnotesize
\tabcolsep=0.11cm
\begin{tabular}{l|ll|ll|ll|ll|ll|ll|ll|ll}
\hline
\multirow{2}{*}{\textbf{Scope}} & 
\multicolumn{2}{c}{\textbf{CodeQL}} & 
\multicolumn{2}{c}{\textbf{NodeJsScan}} & 
\multicolumn{2}{c}{\textbf{ESLint SSC}} &
\multicolumn{2}{c}{\textbf{Graudit}} &
\multicolumn{2}{c}{\textbf{InsiderSec}} &
\multicolumn{2}{c}{\textbf{MS DevSkim}} &
\multicolumn{2}{c}{\textbf{Drek}} &
\multicolumn{2}{c}{\textbf{Mosca}} \\
& TP (\%)    & P (\%) & TP (\%)   & P (\%) & TP (\%)    & P (\%) & TP (\%)    & P (\%) & TP (\%) & P (\%) & TP (\%)   & P (\%) & TP (\%) & P (\%) & TP (\%)  & P (\%) \\ \hline
CWE-22    & \cellcolor{green!15}110 (74.8)  & \cellcolor{green!15}90.2  & \cellcolor{yellow!15}59 (40.1) & \cellcolor{yellow!15}69.4 & \cellcolor{green!15}114 (77.6)  & \cellcolor{green!15}88.4  & \cellcolor{green!15}126 (85.7)  & \cellcolor{green!15}88.1  & 1 (0.7) & 5.6    & 0 (0.0)                       & 0.0                      & 0 (0.0)  & 0.0    & 0 (0.0)                       & 0.0                       \\
CWE-79    & \cellcolor{yellow!15}25 (29.1)  & \cellcolor{yellow!15}37.3 & 5 (5.8)                        & 9.6                       & \cellcolor{yellow!15}26 (30.2)  & \cellcolor{yellow!15}40.0 & 11 (12.8)                       & 15.3                      & 0 (0.0) & 0.0    & 0 (0.0)                       & 0.0                      & 0 (0.0)  & 0.0    & 1 (1.2)                       & 1.6                       \\
CWE-818   & \cellcolor{yellow!15}18 (21.4)  & \cellcolor{yellow!15}47.4 & 0 (0.0)                        & 0.0                       & 1 (1.2)                         & 1.4                       & 3 (3.6)                         & 5.6                       & 1 (1.2) & 7.7    & \cellcolor{green!15}70 (83.3) & \cellcolor{green!15}94.6 & 0 (0.0)  & 0.0    & 0 (0.0)                       & 0.0                       \\
CWE-400   & 8 (12.1)                        & 38.1                      & 2 (3.0)                        & 7.7                       & \cellcolor{yellow!15}28 (42.4)  & \cellcolor{yellow!15}52.8 & 4 (6.1)                         & 8.7                       & 0 (0.0) & 0.0    & 0 (0.0)                       & 0.0                      & 0 (0.0)  & 0.0    & 0 (0.0)                       & 0.0                       \\
CWE-471   & \cellcolor{yellow!15}16 (32.0)  & \cellcolor{yellow!15}76.2 & 0 (0.0)                        & 0.0                       & \cellcolor{green!15}39 (78.0)   & \cellcolor{green!15}88.6  & 0 (0.0)                         & 0.0                       & 0 (0.0) & 0.0    & 0 (0.0)                       & 0.0                      & 0 (0.0)  & 0.0    & 0 (0.0)                       & 0.0                       \\
CWE-78    & \cellcolor{green!15}34 (77.3)   & \cellcolor{green!15}91.9  & 3 (6.8)                        & 17.6                      & \cellcolor{yellow!15}17 (38.6)  & \cellcolor{yellow!15}44.7 & 5 (11.4)                        & 16.1                      & 1 (2.3) & 20.0   & 0 (0.0)                       & 0.0                      & 2 (4.5)  & 18.2   & 2 (4.5)                       & 11.1                      \\
CWE-94    & \cellcolor{yellow!15}4 (17.4)   & \cellcolor{yellow!15}36.4 & 2 (8.7)                        & 22.2                      & \cellcolor{green!15}13 (56.5)   & \cellcolor{green!15}65.0  & \cellcolor{yellow!15}6 (26.1)   & \cellcolor{yellow!15}33.3 & 2 (8.7) & 22.2   & 0 (0.0)                       & 0.0                      & 3 (13.0) & 33.3   & 3 (13.0)                      & 23.1                      \\
CWE-20    & 3 (12.5)                        & 50.0                      & 0 (0.0)                        & 0.0                       & \cellcolor{green!15}14 (58.3)   & \cellcolor{green!15}66.7  & 3 (12.5)                        & 16.7                      & 0 (0.0) & 0.0    & 0 (0.0)                       & 0.0                      & 1 (4.2)  & 33.3   & 1 (4.2)                       & 7.7                       \\
CWE-200   & \cellcolor{yellow!15}2 (15.4)   & \cellcolor{yellow!15}40.0 & 0 (0.0)                        & 0.0                       & \cellcolor{yellow!15}2 (15.4)   & \cellcolor{yellow!15}22.2 & 1 (7.7)                         & 9.1                       & 1 (7.7) & 50.0   & 1 (7.7)                       & 20.0                     & 0 (0.0)  & 0.0    & 0 (0.0)                       & 0.0                       \\
CWE-89    & 0 (0.0)                         & 0.0                       & \cellcolor{yellow!15}3 (27.3)  & \cellcolor{yellow!15}42.9 & \cellcolor{yellow!15}2 (18.2)   & \cellcolor{yellow!15}20.0 & \cellcolor{yellow!15}5 (45.5)   & \cellcolor{yellow!15}45.5 & 0 (0.0) & 0.0    & 1 (9.1)                       & 16.7                     & 0 (0.0)  & 0.0    & \cellcolor{yellow!15}5 (45.5) & \cellcolor{yellow!15}45.5 \\
Other CWE & \cellcolor{yellow!15}39 (19.8)  & \cellcolor{yellow!15}40.2 & 21 (10.7)                      & 20.8                      & \cellcolor{yellow!15}48 (24.4)  & \cellcolor{yellow!15}29.6 & \cellcolor{yellow!15}32 (16.2)  & \cellcolor{yellow!15}18.8 & 1 (0.5) & 2.0    & 9 (4.6)                       & 7.8                      & 3 (1.5)  & 7.3    & 4 (2.0)                       & 3.4                       \\ \hline
Dataset   & \cellcolor{yellow!15}259 (34.8) & \cellcolor{yellow!15}60.1 & 95 (12.8)                      & 28.2                      & \cellcolor{yellow!15}304 (40.8) & \cellcolor{yellow!15}48.9 & \cellcolor{yellow!15}196 (26.3) & \cellcolor{yellow!15}33.2 & 7 (0.9) & 4.8    & 81 (10.9)                     & 21.8                     & 9 (1.2)  & 5.1    & 16 (2.1)                      & 4.3                       \\
\hline
\end{tabular}
\caption{\small TPR and Precision for each tool by: Path Traversal (CWE-22), Cross-site Scripting (CWE-79), Insufficient Transport Layer Protection (CWE-818), Resource Exhaustion (CWE-400), Modification of Assumed-Immutable Data (CWE-471), OS Command Injection (CWE-78), Code Injection (CWE-94), Improper Input Validation (CWE-20), Exposure of Sensitive Information (CWE-200), and SQL Injection (CWE-89).}
\label{table:raw-detection}
\vspace{-0.5cm}
\end{table*}
